Learning from My Partner's Actions: Roles in Decentralized Robot Teams

When teams of robots collaborate to complete a task, communication is often necessary. Like humans, robot teammates should implicitly communicate through their actions: but interpreting our partner's actions is typically difficult, since a given action may have many different underlying reasons. Here we propose an alternate approach: instead of not being able to infer whether an action is due to exploration, exploitation, or communication, we define separate roles for each agent. Because each role defines a distinct reason for acting (e.g., only exploit, only communicate), teammates now correctly interpret the meaning behind their partner's actions. Our results suggest that leveraging and alternating roles leads to performance comparable to teams that explicitly exchange messages. You can find more images and videos of our experimental setups at http://ai.stanford.edu/blog/learning-from-partners/.

==> notes.tex <==
\section{Interpreting Actions via Roles}

Consider a decentralized, two-agent team where the agents share a common objective. Each agent observes part of the system state. If the agents could explicitly convey these observations to their partner, the team could follow a centralized policy. But our agents cannot explicitly convey information; instead, they \textit{implicitly} communicate through \textit{actions}. In this section, we show that interpreting the meaning behind another agent's action is challenging. Recall the table moving example: when our partner applies a force, how do we know which components of that force are meant to (a) move the team towards the goal, (b) communicate about potential obstacles, or (c) respond to our own actions? Each agent must reason over their partner's behavior, and this behavior may in turn depend on the first agent's actions. We introduce speaker and listener roles to break this recursion, so that teammates can correctly interpret the implicit communication within their partner's actions.

\textbf{Jointly Fully Observable.} Throughout this work we assume that the system state is jointly fully observable. In other words, the system state is uniquely determined when we are given the current observations of both teammates.

\textbf{MMDP.} Let us start with teams that \textit{explicitly} communicate, so that each teammate transmits their observations directly to their partner. Since the state is jointly fully observable, explicit communication results in teams where both agents know the state. We formalize this setting as a (factored) multi-agent Markov decision process (MMDP): $\mathcal{M}_E = \langle \alpha, \{\mathcal{S}_i\}_{i \in \alpha}, \{A_i\}_{i \in \alpha}, T, R, h \rangle$.
Here $\alpha$ is the discrete set of agents, $\mathcal{S}_i$ is the state space for agent $i$, $\mathcal{A}_i$ is the action space for agent $i$, $T : \mathcal{S} \times \mathcal{A} \times \mathcal{S} \rightarrow [0,1]$ is the team transition model, $R : \mathcal{S} \times \mathcal{A} \rightarrow \mathbb{R}^+$ is the reward function, and $h$ is the time horizon. For two-player teams, the system state at timestep $t$ is $s^t = (s_1^t,s_2^t)$, the joint action is $a^t = (a_1^t,a_2^t)$, and the optimal policies are $\pi_1^*(a_1^t~|~s_1^t,s_2^t)$ and $\pi_2^*(a_2^t~|~s_1^t,s_2^t)$.

\textbf{Dec-MDP.} We are interested in teams that \textit{implicitly} communicate through actions, but cannot directly convey their observations to their teammate. We formalize this setting as a (factored) decentralized Markov decision process (Dec-MDP): $\mathcal{M}_I = \langle \alpha, \{\mathcal{S}_i\}_{i \in \alpha}, \{A_i\}_{i \in \alpha}, T, R, \{\Omega_i\}_{i \in \alpha}, O, h \rangle$. Here $\Omega_i$ is the observation space for agent $i$ and $O : \Omega \times \mathcal{S} \rightarrow [0,1]$ is the team observation model. The $i$-th agent observes its own state component $s_i^t$ and the team collectively observes $o^t = (s_1^t,s_2^t)$. Let $s_i^{0:t}$ be the history of observations for agent $i$ and let $a^{0:t}$ be the history of actions. Agents in Dec-MDPs make decisions based on these histories: $\pi_1(a_1^t ~|~ s_1^{0:t}, a^{0:t})$ and $\pi_2(a_2^t ~|~ s_2^{0:t}, a^{0:t})$. 

\textbf{Matching Explicit Behavior.} Solving a Dec-MDP for the optimal behavior of each agent is NEXP-complete, while solving an MMDP is P-complete. Because we can tractably solve the MMDP, we will focus on controlling our implicitly communicating agents to match the behavior of a team with explicit communication. The implicitly communicating agents have policies $\pi_i(a_i^t|s_i^{0:t},a^{0:t})$, and we want these policies to match the explicit communication policies $\pi_i^*(a_i^t~|~s_1^t,s_2^t)$. When both agents choose their policy to best match the explicit behavior, we reach:
\begin{equation} \label{eq:recur1}
    \pi_1(a_1^t~|~s_1^{0:t},a^{0:t}) \propto \sum_{s_2^{0:t}} \pi_1^*(a_1^t~|~s_1^t,s_2^t) \cdot \pi_2(a_2^t~|~s_2^{0:t},a^{0:t}) \cdot P(s_2^{0:t}~|~s_1^{0:t},a^{0:t-1})
\end{equation}
\begin{equation} \label{eq:recur2}
    \pi_2(a_2^t~|~s_2^{0:t},a^{0:t}) \propto \sum_{s_1^{0:t}} \pi_2^*(a_2^t~|~s_1^t,s_2^t) \cdot \pi_1(a_1^t~|~s_1^{0:t},a^{0:t}) \cdot P(s_1^{0:t}~|~s_2^{0:t},a^{0:t-1})
\end{equation}
The first term (on the right side) is the behavior that the agent is trying to emulate, the second term is the partner's policy, and the third term is the agent's current belief over the unobserved state. 

\textbf{Interpreting Actions.} Solving (\ref{eq:recur1}) and (\ref{eq:recur2}) leads to infinite recursion, and, at each level of recursion, the agents must marginalize over the state history. We recognize that leveraging implicit communication is challenging: it is hard for agents to correctly interpret the meaning behind their partner's actions because agents have to reason about what their partner is thinking they are thinking, etc. We break this infinite recursion by introducing speaker and listener roles.

\textbf{Speaker.} We define a \textit{speaker} as an agent that makes decisions based only on its private information (e.g., the observations $s_i^{0:t}$). Let agent $1$ be the speaker; the speaker policy that best matches $\pi_1^*$ is:
\begin{equation} \label{eq:speaker}
    \pi_1(a_1^t~|~s_1^{0:t}) = \sum_{s_2} \pi_1^*(a_1^t ~|~ s_1^t,s_2^t) \cdot P(s_2^t~|~s_1^{0:t})
\end{equation}
More generally, any policy of the form $\pi_i(a_i^t~|~s_i^{0:t})$ is a speaker. Because speakers take actions predicated only on their private information, their actions convey this private information to teammates.

\textbf{Listener.} We define a \textit{listener} as an agent that makes decisions based both on its private information and the partner's actions, and models the partner as a speaker. If agent $2$ is the listener, the listener policy that best matches $\pi_2^*$ is:
\begin{equation} \label{eq:listener}
    \pi_2(a_2^t~|~s_2^{0:t},a^{0:t}) \propto \sum_{s_1^{0:t}} \pi_2^*(a_2^t~|~s_1^t,s_2^t) \cdot \pi_1(a_1^t~|~s_1^{0:t}) \cdot P(s_1^{0:t}~|~s_2^{0:t},a^{0:t-1})
\end{equation}
More generally, any policy of the form $\pi_i(a_i^t~|~s_i^{0:t},a^{0:t})$ is a listener if it interprets its teammates actions with $\pi_j(a_j^t~|~s_j^{0:t})$, where $i \neq j$. Listeners can interpret the meaning of speaker actions, and leverage their partner's actions to gain information about the unobserved state. 

\textbf{Roles.} We introduced roles so that agents can effectively communicate through their actions. Comparing the speaker-listener team (\ref{eq:speaker})--(\ref{eq:listener}) to our original team (\ref{eq:recur1})--(\ref{eq:recur2}), we have now removed the infinite recursion over actions. Intuitively, roles provide a directed information exchange from speakers to listeners. We will explore how these roles should be used to make teams that implicitly communicate mimic explicitly communicating teams. However, we emphasize that these roles are more generally defined: they cover two classes of policies that are conditioned on different types of information, and may therefore be applicable for communicating in other decentralized control tasks.

\section{Analyzing Roles in Linear Feedback Systems}

We have introduced speaker and listener roles for decentralized teams, and discussed how these roles enable agents to convey and interpret implicit communication. We are interested in leveraging these roles to mimic the behavior of explicitly communicating teams. In this section we explore a specific case, where the system has continuous-time dynamics, and the explicitly communicating team follows a linear feedback policy with additive white Gaussian noise. This case could correspond to settings where the MMDP is a linear-quadratic regulator (LQR). Focusing on linear feedback systems enables us to formally analyze how teams should assign and dynamically change roles, as well as what policies agents should follow within those roles.

\textbf{Linear Feedback.} Let the solution to the MMDP be a feedback control law: $a^t = -K^ts^t + n^t$. Here $K \in \mathbb{R}^{2 \times 2}$ is a feedback gain matrix, and $n \sim \mathcal{N}(\cdot ~|~0, W)$ is zero-mean Gaussian noise with variance $W = diag(w_1^2, w_2^2)$. Hence, the explicitly communicating agents follow the policies:
\begin{equation} \label{eq:lopt1}
    \pi_1^*(a_1^t ~|~ s_1^t, s_2^t) = \mathcal{N}(a_1^t~|-K_{11}^ts_1^t - K_{12}^ts_2^t, w_1^2)
\end{equation}
\begin{equation} \label{eq:lopt2}
    \pi_2^*(a_2^t ~|~ s_1^t, s_2^t) = \mathcal{N}(a_2^t~|-K_{21}^ts_1^t - K_{22}^ts_2^t, w_2^2)
\end{equation}
When the variance is zero these policies become deterministic, so that $a_1^t = -K_{11}^ts_1^t - K_{12}^ts_2^t$ and $a_2^t = -K_{21}^ts_1^t - K_{22}^ts_2^t$. In what follows, we attempt to mimic these policies by leveraging roles.

\subsection{Theoretical Results: Who Should Speak and How?}

\textbf{Fixed Roles.} When both teammates have fixed role allocations, the closed-loop system can become unstable for any choice of feedback gain $K$. This not only included cases where one agent is always the speaker and the other is always a listener, but also cases where both agents are speakers or both agents are listeners.

\textbf{Dynamic Roles.} Let the agents alternate between speaker and listener roles with frequency $\omega$. As $\omega \rightarrow \infty$, we can select speaker and listener behavior such that the implicitly communicating team converges to the policy of the explicitly communicating team in expectation.

\textbf{Communication.} Let $\sigma_i^2$ be the variance of the speaker's policy, and let $\sigma_j^2$ be the variance of the listener's policy. The speaker and listener policies that minimize the KL divergence between the explicitly and implicitly communicating teams have variance:
\begin{equation} \label{eq:var}
    \sigma_i^2 = \frac{K_{ii}^2w_i^2w_j^2}{K_{ii}^2w_j^2 + K_{ji}^2w_i^2}, \quad \sigma_j^2 = w_j^2
\end{equation}
Hence, the speaker should follow a less stochastic (i.e., more communicative) policy than the corresponding desired policy if the listener's actions depend on the speaker's state.

\subsection{Proofs and Extensions to $N$-Agent Teams}

\textbf{Fixed Roles.} We show examples where the fixed-role allocations lead to instability in controllable linear time-invariance systems. Let the team have dynamics $\dot{s} = As + Ba$, where $A,B \in \mathbb{R}^{2\times2}$, and $rank(\begin{bmatrix}B& AB\end{bmatrix}) = 2$. For a feedback controller $a = -Ks + n$, the closed-loop system is stable if and only if all of the eigenvalues of $A - BK$ have a strictly negative real part.

\textit{Speaker-Speaker.} In this role allocation, both agents make decisions based only on their own private information: $a_1 = -K_{11}s_1 + n_1$ and $a_2 = -K_{22}s_2 + n_2$. Consider the example where $A = I_2$ and $B = \mathbbm{1}_{2\times2} - I_2$. For this example the eigenvalues are: $1 \pm \sqrt{K_{11}K_{22}}$, and thus the closed-loop system has a positive eigenvalue (i.e., is unstable) for any choice of speaker gains $K_{11}$ and $K_{22}$.

\textit{Speaker-Listener.} Let agent $1$ always be the speaker and let agent $2$ be the listener. The listener infers the speaker's state $s_1$ from $a_1$, and takes actions $a_2 = -K_{21}s_1-K_{22}s_2 + n_2 + K_{21}K_{11}^{-1}n_1$. Consider an example where $A = \begin{bmatrix} 1 & 1 \\ 0 & 1 \end{bmatrix}$ and $B = \begin{bmatrix} 0 & 0 \\ 1 & 0 \end{bmatrix}$. For this example the eigenvalues are: $1 \pm \sqrt{-K_{11}}$, and thus the closed-loop system has a positive eigenvalue (i.e., is unstable) for any choice of speaker and listener gains $K_{11}$, $K_{21}$, and $K_{22}$.

\textit{Listener-Listener.} Each agent incorrectly models their teammate as a speaker. When $K_{12} \neq 0$ or $K_{21} \neq 0$, this leads to agents that estimate their partner's state has having infinite magnitude. Hence, the team's control actions are also infinite magnitude, and the system is unstable.

\textbf{Dynamic Roles.} We know that fixed roles can fail---but what about teams where agents switch back and forth between speaker and listener roles with frequency $\omega$? Select the speaker and listener policies so that the team takes actions $a_{S1}$ and $a_{S2}$ when agent $1$ or $2$ is the speaker, respectively:
\begin{equation}
    a_{S1} = -\begin{bmatrix} K_{11} & 0 \\ 2K_{21} & K_{22} \end{bmatrix}s + \begin{bmatrix} n_1 \\ n_2 + 2\frac{K_{21}}{K_{11}}n_1 \end{bmatrix}, \quad a_{S2} = -\begin{bmatrix} K_{11} & 2K_{12} \\ 0 & K_{22} \end{bmatrix}s + \begin{bmatrix} n_1 + 2\frac{K_{12}}{K_{22}}n_2 \\ n_2 \end{bmatrix}
\end{equation}
As $\omega \rightarrow \infty$, the team's action approaches the average of $a_{S1}$ and $a_{S2}$:
\begin{equation}
    a_{\omega \rightarrow \infty} = \frac{1}{2}(a_{S1} + a_{S2}) = -Ks + \begin{bmatrix} n_1 + K_{12}K_{22}^{-1}n_2 \\ n_2 + K_{21}K_{11}^{-1}n_1 \end{bmatrix}
\end{equation}
Recalling that the noise $n_1$ and $n_2$ is zero-mean, $\mathbb{E}[a_{\omega \rightarrow \infty}] = -Ks$. Hence, the expected behavior of our team with implicit communication matches the expected behavior of the explicitly communicating team. We note that the noise is amplified by observing the partner's actions.

\textbf{Communication.} Alternating between speaker and listener roles matches the explicitly communicating policy in expectation; but how should agents choose their speaker or listener behavior itself? Here we focus on the variance of these policies. Let agent $1$ be the speaker with policy $\pi_1 = \mathcal{N}(a_1^t~|~-K_{11}^ts_1^t, \sigma_1^2)$ and let agent $2$ be the listener with policy $\pi_2 = \mathcal{N}(a_2^t~|~-K_{21}^ts_1^t - K_{22}^ts_2^t, \sigma_2^2)$. We want to select $\sigma_1^2$ and $\sigma_2^2$ to minimize the KL divergence between these policies and (\ref{eq:lopt1})--(\ref{eq:lopt2}):
\begin{equation}
    \min_{\sigma_1^2, \sigma_2^2} D_{KL}(\pi_1 \| \pi_1^*) + D_{KL}(\pi_2 \| \pi_2^*)
\end{equation}
Taking the expectation of this KL divergence between two normal distributions, we reach:
\begin{equation}
    \min_{\sigma_1^2, \sigma_2^2} \bigg[ \log{\frac{w_1w_2}{\sigma_1\sigma_2}} + \frac{\sigma_1^2}{2w_1^2} + \frac{\sigma_2^2 +  K_{21}^{2}\sigma_1^2/K_{11}^{2}}{2w_2^2}\bigg]
\end{equation}
The variances given in (\ref{eq:var}) minimize this expression. Although the listener can greedily match the variance of the desired policy, the speaker must compromise between matching the variance of the desired policy and reducing its variance to effectively communicate with the listener.

\textbf{$N$-Agent Teams.} Moving beyond two-agent teams, our findings also apply to $N$-agent teams that are attempting to follow a linear feedback policy. Here one agent is the speaker, and $N-1$ agents listen to that speaker. When the agents cycle the speaker role with frequency $\omega$, the action approaches $\frac{1}{N}(a_{S1} + a_{S2} + \ldots + a_{SN})$. As in the two-agent case, we can solve for the control gains and variance to mimic the explicitly communicating team.

\section{Analyzing Roles in Linear Feedback Systems}

Now that we have introduced roles for decentralized teams, we will explore how these roles operate in teams with linear time-invariant (LTI) dynamics. We focus on cases where the coordinated policy is a linear-quadratic regulator (LQR), and we identify sufficient conditions for matching coordinated LQR performance on fully distributed teams. When the team has fixed, pre-defined roles, there exist controllable dynamics such that team becomes unstable for any choice of speaker or listener policies. By contrast, agents that alternate between speaker and listener roles can match the coordinated LQR performance on any controllable LTI system. These results hold in expectation when the observation noise over a teammate's action is unbiased, and also extend to $N$ agent teams.

\textbf{LTI Systems.} Let the two-agent team have continuous-time dynamics $\dot{s} = As + Ba$, where:
\begin{equation}
    \begin{bmatrix} \dot{s}_1(t) \\ \dot{s}_2(t) \end{bmatrix} = \begin{bmatrix} A_{11} & A_{12} \\ A_{21} & A_{22} \end{bmatrix}\begin{bmatrix} s_1(t) \\ s_2(t) \end{bmatrix} + \begin{bmatrix} B_{11} & B_{12} \\ B_{21} & B_{22} \end{bmatrix}\begin{bmatrix} a_1(t) \\ a_2(t) \end{bmatrix}
\end{equation}
We assume that the system is controllable, so that $rank(\begin{bmatrix}B& AB\end{bmatrix}) = 2$. The coordinated LQR policy is a full state feedback controller: $a = -Ks$. In what follows, we attempt to match the performance of this coordinated LQR policy with fixed and dynamic role allocations.

\subsection{Fixed Roles Can Result in Unstable Teams}

Here we consider teams with three different fixed role allocations: speaker-speaker, speaker-listener, and listener-listener. We show that each of these fixed role allocations can fail: there exist dynamics where the decentralized robot team becomes unstable for any choice of feedback controller.

\textbf{Speaker-Speaker.} Both agents make decisions based only on their own observed state:
\begin{equation}
    \begin{bmatrix} a_1(t) \\ a_2(t) \end{bmatrix} = -\begin{bmatrix} K_{11} & 0 \\ 0 & K_{22} \end{bmatrix}\begin{bmatrix} s_1(t) \\ s_2(t) \end{bmatrix}
\end{equation}
There exist dynamics where this controller is unstable for any choice of $K_{11}$ and $K_{22}$. For instance:
\begin{equation}
    A = \begin{bmatrix} 1 & 0 \\ 0 & 1 \end{bmatrix}, \quad B = \begin{bmatrix} 0 & 1 \\ 1 & 0 \end{bmatrix}, \quad \lambda = 1 \pm \sqrt{K_{11}K_{22}}
\end{equation}
where $\lambda$ are the eigenvalues of the closed-loop matrix $A - BK$. In order for this system to be stable, both eigenvalues $\lambda$ must be negative; however, for any choice of $K_{11}$ and $K_{22}$ at least one eigenvalue is positive, and so the team of speakers fails.

\textbf{Speaker-Listener.} Let agent $1$ be the speaker and let agent $2$ be the listener. The listener infers the speaker's state by observing their action selection: $s_1 = -K_{11}^{-1}a_1$. Hence, the controller is:
\begin{equation}
    \begin{bmatrix} a_1(t) \\ a_2(t) \end{bmatrix} = -\begin{bmatrix} K_{11} & 0 \\ K_{21} & K_{22} \end{bmatrix}\begin{bmatrix} s_1(t) \\ s_2(t) \end{bmatrix}
    \label{eq:s-l-controller}
\end{equation}
There exist controllable systems where the fixed speaker-listener roles fail, such as:
\begin{equation}
    A = \begin{bmatrix} 1 & 1 \\ 0 & 1 \end{bmatrix}, \quad B = \begin{bmatrix} 0 & 0 \\ 1 & 0 \end{bmatrix}, \quad \lambda = 1 \pm \sqrt{-K_{11}}
\end{equation}
As before, $\lambda$ are the eigenvalues of the closed-loop matrix $A - BK$, and one of these eigenvalues is positive regardless of the choice of $K_{11}$. This team is unstable for any controller gains.

\textbf{Listener-Listener.} Each agent (incorrectly) models their teammate as a speaker. Let $\hat{s}_1 = -K_{11}^{-1}a_1$ be the second agent's estimate of $s_1$, and let $\hat{s}_2 = -K_{22}^{-1} a_2$ be the first agent's estimate of $s_2$. When $K_{12}, K_{21} \neq 0$, this leads to infinite recursion: $\hat{s_1} = s_1 + K_{11}^{-1}K_{12}\hat{s}_2$ and $\hat{s_2} = s_2 + K_{22}^{-1}K_{21}\hat{s}_1$. Accordingly, teams composed of only listeners become unstable for any $K_{12}, K_{21} \neq 0$, since each agent's estimate of the other's state goes to infinity, and thus the control effort also goes to infinity.

\subsection{Dynamic Role Switching Converges to Coordinated LQR Performance}

\begin{figure}[t]

	\begin{center}
		\includegraphics[width=1.0\columnwidth]{Figures/example1.pdf}

		\caption{Dynamic role switching matches coordinated LQR control. As we increase the frequency that the agents alternate between speaker and listener roles, our team performance converges to the LQR solution (Left, gray is the LQR behavior). This dynamic role switching is robust to zero mean Gaussian noise over the partner's actions (Middle), and can scale to teams of $N$ agents (Right).}

		\label{fig:example1}
	\end{center}

\vspace{-1em}

\end{figure}

We know that fixed roles can fail---but what about teams where agents have dynamic roles? Here we consider a simple dynamic role allocation strategy, where the agents alternate between the speaker and listener roles at a pre-defined frequency. We show that this simple switching strategy is enough to mimic coordinated LQR performance, with extensions for noisy actions and $N$-agent teams.

\textbf{Alternating Roles.} Consider a simple role adaptation strategy where the robots switch back and forth between speaker-listener and listener-speaker roles at a fixed frequency:
\begin{equation}
    a(t) = \begin{cases} K_1 & \text{if $\sin(\omega t) > 0$} \\ K_2 & \text{otherwise} \end{cases}, \quad K_1 = \begin{bmatrix} K_{11} & 0 \\ K_{21} & K_{22} \end{bmatrix}, \quad K_2 = \begin{bmatrix} K_{11} & K_{12} \\ 0 & K_{22} \end{bmatrix}
\end{equation}
As $\omega$ increases, the system converges to: $\dot{s} = As - \frac{1}{2}B(K_1 + K_2)s$. By setting $K = \frac{1}{2}(K_1 + K_2)$ and solving for the control gains $K_1$ and $K_2$, we can match the performance of the coordinated LQR controller on any controllable LTI system.

\textbf{Noisy Actions.} So far we have assumed that each agent perfectly observes the actions of their teammate. More generally, the listener (e.g., agent $2$) may observe $a_1 + n_1$, where $n_1$ is some observation noise. In these cases, the listener's estimate of the speaker's state becomes $\hat{s}_1 = s_1 - K_{11}^{-1}n_1$, and the added noise linearly propagates through the controller: $a_2 = -K_{21}s_1 - K_{22}s_2 + K_{21}K_{11}^{-1}n_1$. If we have that the observation noise is unbiased, however, alternating between speaker and listener roles still converges to coordinated LQR performance in expectation: $\mathbb{E}[a_2] = -K_{21}s_1 - K_{22}s_2$.

\textbf{$N$-Agent Teams.} Moving beyond two-agent teams, robots can also alternate between speaker and listener roles in $N$-agent scenarios to obtain coordinated LQR performance. Let one agent be the speaker, and let the other $N-1$ agents listen to this speaker; if the robots alternate the speaker role, then the closed-loop system converges to: $\dot{s} = As - \frac{1}{N} B (\sum_{i \in N} K_i) s$. As in the two-agent case, we can then set $K = \frac{1}{N}\sum_{i \in N} K_i$ and solve for the control gains that mimic the LQR gain.

%\mx{Also we can play with the relative weights of the two $K$ gains by changing how much relative time is spent with each system before switching. This would give us more general form: $\dot{s} = A + B(\alpha K_1 + (1-\alpha)K_2)$, where $\alpha$ controls the ratio of using controller $K_1$ and $1-\alpha$ for controller $K_2$. These results also extend to discrete systems. }

%\mx{Fig. \ref{fig:example1} shows the plots of LQR simulation with different switching frequencies on the system that is unstable for fixed speaker-listener. We could see that with frequency $\omega = 1Hz$, the system oscillates. However, with higher switching frequency of $\omega = 10Hz, 100Hz$, the system could match the centralized policy quite well. It also matches our theoretical analysis that, with infinite high frequency, the switching roles strategy could asymptotically approximate the centralized controller perfectly.}

%\textbf{Does this Extend to $N$ Player Teams?} \mx{Yes, in multi-agent team with n agents ($n\geq 3$), the advantages of dynamic role allocation still preserve. With $n\geq 3$, there are more feasible configurations for a mixed speaker-listener team. We give a simple example of role adaptation strategy to show that dynamic role switching could still solve the problem when $n\geq 3$. }

%\mx{Consider a team with only one listener at each time step. Let $K_i$ denotes the controller when agent $i$ is the listener. $K_i$ would take the form of $K_{pq} = 0$ for entries $p\neq q$ and $p\neq i, q\neq i$, as in Equ.\ref{eq:n_n_matrix}.
%\begin{equation}
%    \begin{bmatrix}
%    K_{11} & 0 & \dots & 0 \\
%    0 & K_{22} & \dots & 0 \\
%    \vdots & \vdots & \ddots & 0\\
%    K_{i1} & K_{i2} & \dots & K_{in} \\
%    \vdots & \vdots & \vdots & \vdots \\
%    0 & 0 & \dots & K_{nn}
%    \end{bmatrix}
%    \label{eq:n_n_matrix}
%\end{equation}
%If we switch sequentially and circularly from $K_1$ to $K_n$ with high frequency. The system approaches:
%\begin{equation}
%    \dot s = As - B(\frac{1}{n}\sum_{i=1}^n K_i)s
%\end{equation}
%Similarly, we could also match the LQR controller of any LTI system by matching matrix $K_{LQR} = \frac{1}{n}\sum_{i=1}^n K_i$. Therefore, the dynamic role strategy also extends to N player teams.
%}

\section{Who Should Speak and How?}

We found that alternating between speaker and listener roles is sufficient to replicate coordinated LQR performance in decentralized, LTI teams. Next, we apply roles to teams with arbitrary dynamics. Given a coordinated policy that these fully distributed agents should match, we ask two related questions: which agent should be the speaker, and what are the best speaker and listener policies? We answer these questions by greedily minimizing the divergence between the coordinated and fully distributed policies. Interestingly, we find that effective speakers take actions that are less stochastic than the coordinated policy; reducing speaker noise enables the listener to better infer the speaker's private information, and improves the overall team performance.

\textbf{Minimizing Divergence.} Recall that the coordinated behavior is given by $\pi_1^*$ and $\pi_2^*$, and we want our team to match this coordinated behavior. We write this as a greedy optimization problem, where at the current timestep $t$ we choose $\pi_1$ and $\pi_2$ according to:
\begin{equation}
\min_{i \in \{1,2\}}\min_{\pi_i, \pi_j} d\big(\pi_i(a_i^t~|~s_i^{0:t}),\pi_i^*(a_i^t~|~s_i^t,s_j^t)\big) + d\big((\pi_j(a_j^t~|~s_j^{0:t},a^{0:t}),\pi_j^*(a_j^t~|~s_i^t,s_j^t)\big)
\end{equation}
Here agent $i$ is the speaker and agent $j \neq i$ is the listener. The outer-loop tells us \textit{who} should speak, while the inner-loop tells us \textit{how} they should speak.
%reorder?
\textbf{Feedback Example.} Consider a case where the coordinated policy is Gaussian:
\begin{equation}
    \pi_1^*(a_1~|~s_1,s_2) = \mathcal{N}(a_1~|~K_{11}s_1 + K_{12}s_2, \sigma_{1,*}^2), \quad \pi_2^*(a_2~|~s_1,s_2) = \mathcal{N}(a_2~|~K_{21}s_1 + K_{22}s_2, \sigma_{2,*}^2)
\end{equation}
WLOG for now let agent $1$ be speaker. The states $s_1$ and $s_2$ are constant and independent, and sampled from Gaussian priors: $\mathcal{N}(s_1~|~\mu_1, \sigma_{s_1}^2)$ and $\mathcal{N}(s_2~|~\mu_2, \sigma_{s_2}^2)$.
\begin{equation}
    \pi_1(a_1~|~s_1) = \mathcal{N}(a_1~|~K_{11}s_1 + K_{12}\mu_2, \sigma_{1}^2)
\end{equation}
\begin{equation}
    \pi_2(a_2~|~s_2,a_1) = \mathcal{N}(a_2~|~K_{21}K_{11}^{-1}(a_1 - K_{12}\mu_2) + K_{22}s_2, \sigma_{2}^2)
\end{equation}
\mx{
additional constraint posed by observation noise:
\begin{equation}
    \sigma_1^2 \geq K_{11}^2\omega_1^2~~~, \sigma_2^2 \geq K_{22}^2\omega_2^2~~~
\end{equation}
}
Now we can do the KL divergence to determine who should speak and how:
\begin{multline}
    \min_{\theta} KL =  \min_{\theta}\bigg[ \log{\frac{\sigma_{1,*}}{\sigma_1}} + \frac{\sigma_1^2 + (K_{11}s_1 + K_{12}s_2 - K_{11}s_1 - K_{12}\mu_2)^2}{2\sigma_{1,*}^2} +  \log{\frac{\sigma_{2,*}}{\sigma_2}} + \\ \frac{\sigma_2^2 + (K_{21}s_1 + K_{22}s_2 - K_{21}K_{11}^{-1}(a_1 - K_{12}\mu_2) - K_{22}s_2)^2}{2\sigma_{2,*}^2}\bigg]
\end{multline}
\begin{equation}
    =  \min_{\theta}\bigg[ \log{\frac{\sigma_{1,*}\sigma_{2,*}}{\sigma_1\sigma_2}} + \frac{\sigma_1^2}{2\sigma_{1,*}^2} + \frac{K_{12}^{2}(s_2 - \mu_2)^2}{2\sigma_{1,*}^2} + \frac{\sigma_2^2 + K_{21}^{2}(s_1 - K_{11}^{-1}(a_1 - K_{12}\mu_2))^2}{2\sigma_{2,*}^2}\bigg]
\end{equation}
\begin{equation}
    \min_{\theta} \mathbb{E}[KL] =  \min_{\theta}\bigg[\frac{K_{12}^{2}\sigma_{s_2}^2}{2\sigma_{1,*}^2} + \log{\frac{\sigma_{1,*}\sigma_{2,*}}{\sigma_1\sigma_2}} + \frac{\sigma_1^2}{2\sigma_{1,*}^2} + \\ \frac{\sigma_2^2 +  K_{21}^{2}\sigma_1^2/K_{11}^{2}}{2\sigma_{2,*}^2}\bigg]
\end{equation}
The first term is important in the outer optimization (who should speak). We solve the inner loop in closed form (how to speak), then try each speaker-listener role in the outer loop (who speaks).

If agent $1$ is the speaker, the optimal choices of $\sigma_1$ and $\sigma_2$ are (and if agent $2$ is the speaker):
\begin{equation}
    \sigma_1 = \frac{K_{11}\sigma_{1,*}\sigma_{2,*}}{\sqrt{K_{11}^2\sigma_{2,*}^2 + K_{21}^2\sigma_{1,*}^2}}, \quad \sigma_2 = \sigma_{2,*} \quad|\quad \sigma_1 = \sigma_{1,*}, \quad \sigma_2 = \frac{K_{22}\sigma_{1,*}\sigma_{2,*}}{\sqrt{K_{12}^2\sigma_{2,*}^2 + K_{22}^2\sigma_{1,*}^2}}
\end{equation}
And the minimum values for the KL divergence are given by:
\begin{equation}
    \frac{K_{12}^{2}\sigma_{s_2}^2}{2\sigma_{1,*}^2} + \log{\frac{\sqrt{K_{11}^2\sigma_{2,*}^2 + K_{21}\sigma_{1,*}^2}}{K_{11}\sigma_{2,*}}} + 1 \quad|\quad
    \frac{K_{21}^{2}\sigma_{s_1}^2}{2\sigma_{2,*}^2} + \log{\frac{\sqrt{K_{12}^2\sigma_{2,*}^2 + K_{22}\sigma_{1,*}^2}}{K_{22}\sigma_{1,*}}} + 1
\end{equation}

% \textbf{Example with solving for optimal policy (just for keeping notes)}
% % \begin{equation}
% %     \pi_1^*(a_1~|~s_1,s_2) = \mathcal{N}(a_1~|~A_{11}^*s_1 + A_{12}^*s_2, \sigma_{1,*}^2)
% % \end{equation}
% % \begin{equation}
% %     \pi_2^*(a_2~|~s_1,s_2) = \mathcal{N}(a_2~|~A_{21}^*s_1 + A_{22}^*s_2, \sigma_{2,*}^2)
% % \end{equation}
% % \begin{equation}
% %     \pi_1(a_1~|~s_1) = \mathcal{N}(a_1~|~A_{11}s_1, \sigma_{1}^2)
% % \end{equation}
% % \begin{equation}
% %     \pi_2(a_2~|~s_2,a_1) = \mathcal{N}(a_2~|~A_{21}A_{11}^{-1}a_1 + A_{22}s_2, \sigma_{2}^2)
% % \end{equation}
% \begin{multline}
%     \min_{\theta} KL =  \min_{\theta}\bigg[ \log{\frac{\sigma_{1,*}}{\sigma_1}} + \frac{\sigma_1^2 + (A_{11}^*s_1 + A_{12}^*s_2 - A_{11}s_1)^2}{2\sigma_{1,*}^2} +  \log{\frac{\sigma_{2,*}}{\sigma_2}} + \\ \frac{\sigma_2^2 + (A_{21}^*s_1 + A_{22}^*s_2 - A_{21}A_{11}^{-1}a_1 - A_{22}s_2)^2}{2\sigma_{2,*}^2}\bigg]
% \end{multline}
% Note that there are actually additional constraints on the policy parameters. And we list them here.
% \begin{itemize}
%     \item the speaker's policy parameter $A_{11}$ shouldn't depend on any private state information ($s_1$ and $s_2$). It should be a pre-specified constant, since this parameter serves as a protocol for communication and is known by both agents in advance.
%     \item the listener's policy parameter $A_{21}$ and $A_{22}$ could only looks at $s_2$ and $a_1$, without direct dependence on $s_1$.
% \end{itemize}
% \begin{multline}
%     \min_{\theta} KL =  \min_{\theta}\bigg[ \log{\frac{\sigma_{1,*}}{\sigma_1}} + \log{\frac{\sigma_{2,*}}{\sigma_2}} + \frac{\sigma_1^2}{2\sigma_{1,*}^2} + \frac{\sigma_2^2}{2\sigma_{2,*}^2} + \frac{(A_{11}^*s_1 + A_{12}^*s_2 - A_{11}s_1)^2}{2\sigma_{1,*}^2} + \\ \frac{(A_{21}^*s_1 + A_{22}^*s_2 - A_{21}A_{11}^{-1}a_1 - A_{22}s_2)^2}{2\sigma_{2,*}^2}\bigg]
% \end{multline}
% Solving for $A_{11}$, $A_{21}$ and $A_{22}$, we have
% \begin{multline}
%     \min_{A_{11},A{21},A{22}} KL =  \min_{\theta}\bigg[\mathbb{E}_{s_1,s_2}[\frac{(A_{11}^*s_1 + A_{12}^*s_2 - A_{11}s_1)^2}{2\sigma_{1,*}^2}] +\\ \mathbb{E}_{a_1}\frac{[(A_{21}^*s_1 - A_{21}^*A_{11}^{-1}a_1) + (A_{21}^*A_{11}^{-1}a_1 + A_{22}^*s_2 - A_{21}A_{11}^{-1}a_1 - A_{22}s_2)]^2}{2\sigma_{2,*}^2}\bigg]
% \end{multline}

% \begin{equation}
%     \mathbb{E}_{s_1,s_2}[\frac{(A_{11}^*s_1 + A_{12}^*s_2 - A_{11}s_1)^2}{2\sigma_{1,*}^2}] = \frac{\mathbb{E}(s_1^2)}{2\sigma_{1,*}^2}A_{11}^2 - \frac{\mathbb{E}(s_1(A_{11}s_1+A_{12}s_2))}{\sigma_{1,*}^2}A_{11} + constant
% \end{equation}
% \begin{multline}
% \mathbb{E}_{a_1}\frac{[(A_{21}^*s_1 - A_{21}^*A_{11}^{-1}a_1) + (A_{21}^*A_{11}^{-1}a_1 + A_{22}^*s_2 - A_{21}A_{11}^{-1}a_1 - A_{22}s_2)]^2}{2\sigma_{2,*}^2} = \\ \mathbb{E}_{a_1}\frac{ (A_{21}^*A_{11}^{-1}a_1 + A_{22}^*s_2 - A_{21}A_{11}^{-1}a_1 - A_{22}s_2)^2}{2\sigma_{2,*}^2} + \frac{A^*_{21}^2}{A_{11}^2}\frac{\sigma_1^2}{2\sigma_2^2}
% \end{multline}

% We can always drive the term $(A_{21}^*A_{11}^{-1}a_1 + A_{22}^*s_2 - A_{21}A_{11}^{-1}a_1 - A_{22}s_2)^2$ to zero by optimizing over $A_{21}$ and $A_{22}$. And then solving for $A_{11}$.

% \begin{equation}
%     A_{11} = argmin~\bigg[\frac{\mathbb{E}(s_1^2)}{2\sigma_{1,*}^2}A_{11}^2 - \frac{\mathbb{E}(s_1(A_{11}s_1+A_{12}s_2))}{\sigma_{1,*}^2}A_{11} + \frac{A^*_{21}^2}{A_{11}^2}\frac{\sigma_1^2}{2\sigma_2^2}\bigg]
% \end{equation}
% Which may not have an analytical solution

\section{Problem Statement}

\subsection{Hypothesis}

\textbf{Communicative Roles.} We outline classes of policies that agents can take to convey their information (\textit{speaker}), interpret information conveyed by its partner through the actions (\textit{listener}), or follow a baseline (\textit{independent}).

\textbf{Fixed Teams.} We hypothesize that teams where agents always maintain a fixed role (e.g., speaker, listener, or independent), can fail to accomplish their task. We also quantify how adding random noise to these fixed policies can improve their performance.

\textbf{Adaptive Teams.} We hypothesize that teams where the agents change roles---for example, so that speakers can become listeners---could communicate information more effectively and thus outperform fixed teams.

\textbf{Role Protocol.} Finally, we attempt to identify optimal ways for robots to change roles within a mutually agreed upon protocol, so that both agents are always aware of the role of their partner.

\section{What Are Roles?}

A role is a class of policies. These policies either only consider private information (\textit{speaker}), reason over the partner's actions (\textit{listener}), or ignore both information and actions altogether (\textit{independent}). Intuitively, a speaker makes decisions based on $z$, a listener makes decisions based on $z$ and $a$, and an independent makes decisions while ignoring $z$ and $a$.

\textbf{Speaker.} The speaker has a belief that is only based on its own observations $z$:
\begin{equation}
    b_s^{t+1}(s) = P(s ~|~ z_s^{0:t}) \propto O_s(z_s^t ~ | ~ s) \cdot b_s^t(s)
\end{equation}
The speaker's policy maps from this belief to actions: $\pi_s (a_s ~|~ b_s)$. Thus, the robot's actions convey information about its observation directly. All policies that are only based on an agent's own local observation fall into this class.

\textbf{Listener.} The listener has a belief that is based on its own observations $z$ and its partner's actions $a$:
\begin{equation}
    b_l^{t+1}(s) = P(s ~|~ z_l^{0:t}, a_s^{0:t}) \propto O_l(z_l^t ~ | ~ s) \cdot \sum_{z^{0:t}} \Big[\pi_s(a_s^t ~ | ~ z_s^{0:t})P(z_s^{0:t} ~ | ~ s)\Big] \cdot b_l^t(s)
\end{equation}
The listener's policy maps from this belief to actions: $\pi_l (a_l ~|~ b_l)$. Importantly, a listener assumes that the partner is a speaker, and knows the speaker's policy. All policies that reason over both its private observation and the other agent's actions (while knowing the other agent's policy) fall into this class.

\textbf{Independent.} An independent robot makes decisions without paying attention to $z$ or $a$. When a robot is an independent, it neither conveys information nor receives information to update its own belief. For example, the policy of following its neighboring agent's action, and the complete random policy would fall into this class. All policies that are irrelevant to both its observations and other actions fall into this class.

\subsection{Why These Roles?}

Each agent has a belief over the system state based on $z_i^{0:t}$ and $a^{0:t}$, so that $b_i^{t+1}(s) = P(s ~|~ z_i^{0:t}, a^{0:t})$. Interpreting the other agents' actions is hard; in the full solution, each agent thinks about what the other agents are thinking about what they are thinking, etc. We simplify the problem by breaking that recursion to enable more effective communication.

Specifically, we look at different levels of simplification and refer to them as different roles.

% \subsection{From Beliefs to Policies}

% Once the agent has its belief (as either a leader or listener) it needs to map this belief to actions. This requires accounting for how the other agents will act during the rest of the task. For simplicity, each agent assumes that the other agents will follow the optimal policy (from their point of view). This results in centralized planning for each agent: $\pi_i(a ~|~ b)$. In practice, each agent solves the POMDP that maps their belief to a system action $a$, and then takes action $a_i$.

\textbf{Example.} Speaker chooses less random action (relationship to exploration).

Here is an example where we get to pick $\sigma_1$ and $\sigma_2$. Agent $1$ should definitely be the speaker.
\begin{equation}
\pi_1^*(a_1~|~s_1,s_2) = \mathcal{N}(a_1~|~s_1, \sigma_{1,*}^2), \quad \pi_2^*(a_2~|~s_1,s_2) = \mathcal{N}(a_2~|~s_1, \sigma_{2,*}^2)
\end{equation}
I look for the policy $\pi_1(a_2~|~s_2,a_1)$ that best matches the optimal policy $\pi_2^*$:
\begin{equation}
    \pi_2(a_2~|~a_1) = \sum_{s_1}\frac{P(a_1~|~s_1,a_2)P(a_2~|~s_1)P(s_1)}{P(a_1)} = \frac{1}{P(a_1)} \mathbb{E}_{s_1} \Big[ P(a_1~|~s_1,a_2)P(a_2~|~s_1)\Big]
\end{equation}
Substitute in the policies; assume speaker follows a normal with variance $\sigma_1^2$:
\begin{equation}
    = \frac{1}{P(a_1)} \mathbb{E}_{s_1} \Big[ \pi_1(a_1~|~s_1)\pi_2^*(a_2~|~s_1)\Big] = \frac{1}{P(a_1)} \mathbb{E}_{s_1} \Big[ \mathcal{N}(a_1~|~s_1, \sigma_1^2)\mathcal{N}(a_2~|~s_1, \sigma_{2,*}^2)\Big]
\end{equation}
I want to make this into a Gaussian so that the KL will be clean. Expand the Normals:
\begin{equation}
    \mathcal{N}(a_1~|~s_1, \sigma_1^2)\mathcal{N}(a_2~|~s_1, \sigma_{2,*}^2) = \frac{1}{2\pi\sigma_1\sigma_{2,*}} \exp \bigg[\frac{-(a_1 - s_1)^2}{2\sigma_1^2} + \frac{-(a_2 - s_1)^2}{2\sigma_{2,*}^2}\bigg]
\end{equation}
\begin{equation}
    = \frac{1}{2\pi\sigma_1\sigma_{2,*}} \exp \bigg[\frac{-(s_1 - a_1)^2}{2\sigma_1^2} + \frac{-(s_1 - a_2)^2}{2\sigma_{2,*}^2}\bigg] = S \cdot \frac{1}{\sqrt{2\pi\sigma^2}}\exp \bigg[\frac{-(s_1 - \mu)^2}{2\sigma^2}\bigg]
\end{equation}
\begin{equation}
    \mu = \frac{a_1\sigma_{2,*}^2 + a_2\sigma_1^2}{\sigma_1^2 + \sigma_{2,*}^2}, \quad \sigma^2 = \frac{\sigma_1^2\sigma_{2,*}^2}{\sigma_1^2 + \sigma_{2,*}^2}, \quad S = \mathcal{N}(a_2~|~a_1, \sigma_1^2 + \sigma_{2,*}^2)
\end{equation}
I think this is all algebra? I looked up some stuff online to check it. Plugging back in:
\begin{equation}
    \pi_2(a_2~|~a_1) = \frac{1}{P(a_1)} \mathbb{E}_{s_1} \Big[\mathcal{N}(a_2~|~a_1, \sigma_1^2 + \sigma_{2,*}^2)\mathcal{N}(s_1~|~\mu, \sigma^2)\Big]
\end{equation}
\mx{? missing additional assumption: uniform prior}
\begin{equation}
    \pi_2(a_2~|~a_1) = \frac{\mathcal{N}(a_2~|~a_1, \sigma_1^2 + \sigma_{2,*}^2)}{P(a_1)} \mathbb{E}_{s_1} \Big[\mathcal{N}(s_1~|~\mu, \sigma^2)\Big] = \frac{\mu \cdot \mathcal{N}(a_2~|~a_1, \sigma_1^2 + \sigma_{2,*}^2)}{P(a_1)}
\end{equation}
Now we have dealt with the $s_1$. But it would still be nice to make this a Gaussian...For the KL to work well we want the mean at $a_1$, but perhaps the variance is incorrect?

I'll ignore this for a second, and assume $\pi_2(a_2~|~a_1) \approx \mathcal{N}(a_2~|~a_1, \sigma_1^2 + \sigma_{2}^2)$. Now we can do some KL divergence! We want to minimize the KL between both distributions and the centralized:
\begin{equation}
    \min_{\sigma_1,\sigma_2}\bigg[ \log{\frac{\sigma_1}{\sigma_{1,*}}} + \frac{\sigma_{1,*}^2}{2\sigma_1^2}\bigg] + \bigg[ \log{\frac{\sqrt{\sigma_1^2 + \sigma_{2}^2}}{\sigma_{2,*}}} + \frac{\sigma_{2,*}^2 + (a_1 - s_1)^2}{2(\sigma_1^2 + \sigma_{2}^2)}\bigg] - 1
\end{equation}
I'm leaving $\sigma_2$ as a free variable. Taking the expectation over $a_1$, we get:
\begin{equation}
    \min_{\sigma_1, \sigma_2}\bigg[ \log{\frac{\sigma_1}{\sigma_{1,*}}} + \frac{\sigma_{1,*}^2}{2\sigma_1^2}\bigg] + \bigg[ \log{\frac{\sqrt{\sigma_1^2 + \sigma_{2}^2}}{\sigma_{2,*}}} + \frac{\sigma_{2,*}^2 + \sigma_1^2}{2(\sigma_1^2 + \sigma_{2}^2)}\bigg] - 1
\end{equation}

\textbf{Another Iteration of the Example.}
\begin{equation}
\pi_1^*(a_1~|~s_1) = \mathcal{N}(a_1~|~s_1, \sigma_{1,*}^2), \quad \pi_2^*(a_2~|~s_1) = \mathcal{N}(a_2~|~s_1, \sigma_{2,*}^2)
\end{equation}
\begin{equation}
\pi_1(a_1~|~s_1) = \mathcal{N}(a_1~|~s_1, \sigma_{1}^2), \quad \pi_2(a_2~|~a_1) = \mathcal{N}(a_2~|~a_1, \sigma_{2}^2)
\end{equation}
\begin{equation}
    \min_{\sigma_1,\sigma_2} KL(\pi_1 \| \pi_1^*) + KL(\pi_2 \| \pi_2^*) =  \min_{\sigma_1,\sigma_2}\bigg[ \log{\frac{\sigma_1}{\sigma_{1,*}}} + \frac{\sigma_{1,*}^2}{2\sigma_1^2} +  \log{\frac{\sigma_2}{\sigma_{2,*}}} + \frac{\sigma_{2,*}^2 + (a_1 - s_1)^2}{2\sigma_{2}^2}\bigg]
\end{equation}
\begin{equation}
    =  \min_{\sigma_1,\sigma_2}\bigg[ \log{\frac{\sigma_1}{\sigma_{1,*}}} + \frac{\sigma_{1,*}^2}{2\sigma_1^2} +  \log{\frac{\sigma_2}{\sigma_{2,*}}} + \frac{\sigma_{2,*}^2 + \sigma_1^2}{2\sigma_{2}^2}\bigg]
\end{equation}
That gives us the desired dependence: the listener's KL divergence is affected by the speaker's noise.
